Testing Cumulative Treatment Effects in Continuous Time with ODE Dynamics and Noisy Observations

We develop a semiparametric continuous time inferential framework for testing cumulative treatment effects, including both immediate and carryover effects. The latent state process is modeled by an ordinary differential equation (ODE) whose drift depends on state and treatment, while the observed data are noisy measurements of this latent state at irregular, multi resolution time points. We define the average treatment effect (ATE) as the difference of expected cumulative outcomes under the always treat and always control policies and establish its identifiability from observational data. More generally, the framework accommodates contrasts between arbitrary deterministic stationary treatment policies, including clinically motivated threshold policies, with the always treat versus never treat comparison as the leading special case. A two step estimation procedure first recovers the latent state trajectories and their derivatives via spline smoothing, then solves a continuous time estimating equation derived from the infinitesimal generator of the ODE. We prove asymptotic normality of the resulting test statistic under explicit rate conditions on the spline estimator. The resulting test admits asymptotically valid inference under noisy, irregularly sampled observations, providing a studentized statistic with a standard $N(0,1)$ limit. Simulations show that the proposed method demonstrates improved stability and power over discrete time alternatives in noisy and multi resolution settings, with comparable performance under clean regular grids. We apply the method to the OhioT1DM diabetes dataset to evaluate cumulative effects of insulin treatments on glucose levels.

==> main_labels.tex <==
\newlabel{sec:introduction}{{1}{2}{Introduction}{section.1}{}}
\newlabel{sec:background}{{2}{5}{Background and Notations}{section.2}{}}
\newlabel{eq:ode}{{1}{5}{Background and Notations}{equation.1}{}}
\newlabel{eq:obs}{{2}{6}{Background and Notations}{equation.2}{}}
\newlabel{eq:generator}{{3}{6}{Background and Notations}{equation.3}{}}
\newlabel{sec:methodology}{{3}{7}{Methodology}{section.3}{}}
\newlabel{eq:ate_policy}{{4}{8}{Identification of stationary policy contrasts}{equation.4}{}}
\newlabel{eq:th1}{{5}{8}{Identification of stationary policy contrasts}{equation.5}{}}
\newlabel{alg:test}{{1}{13}{Test procedure}{algocf.1}{}}
\newlabel{sec:theory}{{4}{14}{Theory}{section.4}{}}
\newlabel{thm:bellman}{{4.1}{14}{}{theorem.4.1}{}}
\newlabel{eq:bellman_policy}{{6}{15}{}{equation.6}{}}
\newlabel{eq:spline_rate}{{7}{16}{Asymptotic properties}{equation.7}{}}
\newlabel{thm:normal}{{4.2}{16}{}{theorem.4.2}{}}
\newlabel{sec:discretization}{{4.3}{17}{Discretization bias of discrete-time estimators}{subsection.4.3}{}}
\newlabel{eq:discrete_moment}{{8}{17}{Discretization bias of discrete-time estimators}{equation.8}{}}
\newlabel{thm:discretization}{{4.3}{18}{Discretization and noise-amplification bias}{theorem.4.3}{}}
\newlabel{sec:simulation}{{5}{19}{Numerical Study}{section.5}{}}
\newlabel{sim0}{{9}{21}{Univariate simulations}{equation.9}{}}
\newlabel{fig:treat}{{1}{22}{Treatment schedules used in the one dimensional simulation: Treatment 1 (short period; orange, dashed) and Treatment 2 (long period; blue, solid)}{figure.1}{}}
\newlabel{tb:sim1}{{1}{22}{Test power and Type-I error of competing methods under different treatment assignments and observation noise levels $\epsilon $}{table.1}{}}
\newlabel{sim1}{{10}{24}{Multivariate simulations}{equation.10}{}}
\newlabel{sim2}{{11}{24}{Multivariate simulations}{equation.11}{}}
\newlabel{sim3}{{12}{24}{Multivariate simulations}{equation.12}{}}
\newlabel{tb:sim4}{{2}{25}{Power of competing methods across multivariate settings at treatment effect $\delta =0.05$}{table.2}{}}
\newlabel{tb:policy_sim}{{3}{26}{Policy contrast estimand: rejection rates of the proposed test}{table.3}{}}
\newlabel{sec:realdata}{{6}{27}{Real Data Application}{section.6}{}}
\newlabel{fig:state}{{2}{27}{OhioT1DM multi resolution structure for one patient over 24 hours. Left: state channels, with physiological signals at 1 minute resolution and CGM glucose every 5 minutes. Right: CGM outcome and irregularly timed basal and bolus insulin events}{figure.2}{}}
\newlabel{sec:realdata-bolus}{{6.1}{28}{Bolus insulin: a descriptive cumulative timing association}{subsection.6.1}{}}
\newlabel{tb:realdata}{{4}{29}{Bolus insulin: observed dosing regime versus never dosing (descriptive contrast). Each method is evaluated once on the full data, standardized glucose scale. The t test and clustered OLS share the same contemporaneous estimate and differ only in the variance (iid versus patient clustered $t_{5}$); the proposed cumulative contrast uses the patient clustered variance}{table.4}{}}
\newlabel{sec:realdata-policy}{{6.2}{30}{Basal insulin: comparing two threshold dosing policies}{subsection.6.2}{}}
\newlabel{tb:realdata_policy}{{5}{31}{Basal threshold policies: contrast estimates on the full data with patient clustered $t_{5}$ intervals, leave one patient out (LOPO) ranges, and descriptive subsample rejection frequencies over $50$ day resamples; all estimates use the empirical reference distribution $\mathbb G$, and the per policy overlap diagnostics are collected in Table~\ref {tb:realdata_overlap} of Supplement Section~\ref {sec:realdata-implementation}}{table.5}{}}
\newlabel{sec:discussion}{{7}{32}{Discussion}{section.7}{}}
\newlabel{supplementary-material}{{7}{34}{Declaration of the use of generative AI and AI assisted technologies}{section*.4}{}}

